Predicting 4D Hand Trajectory from Monocular Videos

We present HaPTIC, an approach that infers coherent 4D hand trajectories from monocular videos. Current video-based hand pose reconstruction methods primarily focus on improving frame-wise 3D pose using adjacent frames rather than studying consistent 4D hand trajectories in space. Despite the additional temporal cues, they generally underperform compared to image-based methods due to the scarcity of annotated video data. To address these issues, we repurpose a state-of-the-art image-based transformer to take in multiple frames and directly predict a coherent trajectory. We introduce two types of lightweight attention layers: cross-view self-attention to fuse temporal information, and global cross-attention to bring in larger spatial context. Our method infers 4D hand trajectories similar to the ground truth while maintaining strong 2D reprojection alignment. We apply the method to both egocentric and allocentric videos. It significantly outperforms existing methods in global trajectory accuracy while being comparable to the state-of-the-art in single-image pose estimation. Project website: https://judyye.github.io/haptic-www

==> draft/2_related_work_draft.tex <==
\section{Related Works}
\todo{yy: thanks everyone! Yufei will consolidate it to 1.5 columns}

\input{fig/overview}

% zhang2019HAMR, moon2020i2l, tang2021handAR 
% frankmocap, metro, meshgraphormer, handoccnet, hamer, simplehand, hhmr 
\paragraph{Image-Based Hand Pose Estimation.}
Estimating hand poses from images has been extensively explored, with studies mainly \cite{zhang2019HAMR, moon2020i2l, tang2021handAR, frankmocap} focusing on estimating pose parameters of parametric 3D hand models, such as MANO \cite{mano}. Recently, MeshGraphormer~\cite{metro} introduced a transformer-based approach that outputs mesh vertices for human body and hand meshes based on SMPL~\cite{smpl} and MANO models, combining self-attention from transformers with graph convolutions. HaMeR~\cite{hamer} leverages a large transformer network trained on large-scale datasets to achieve state-of-the-art performance in hand estimation. SimpleHand~\cite{simplehand} provides an efficient solution by using a token generator and mesh regressor to construct a 3D hand mesh. HHMR~\cite{hhmr} proposes a graph diffusion model to learn gesture priors and inpaint occluded hand regions, while Hamba~\cite{hamba} improves performance by capturing spatial joint sequences through a graph-guided state-space model using the Mamba architecture~\cite{Mamba}. These methods perform effectively on single image frames, however, jittering occurs when applied to video sequences. Nonetheless, they establish a solid foundation for video-based hand estimation. \yao{can shortern depends on the space}

% color glove: wang2009real 
% Deformer: Dynamic Fusion Transformer for Robust Hand Pose Estimation: fu2023deformer
% HO3D: optimization 
\paragraph{Video-Based Hand Pose Estimation.} 
Hand tracking has a long history \cite{wang2009real}, with most approaches using multi-view consistency \cite{HO3D,multiviewvideohpe}, depth data \cite{zoe, aerial, liu2022hoi4d, dexycb}, or temporal information from RGB videos. However, relying on extra inputs like IMU or depth can still lead to inaccuracies, since depth data often struggles with heavy self-occlusions. Temporal information is typically used in three main ways: some methods add it as a training constraint to improve pose estimation \cite{hasson2020leveraging, zhou2022toch} for single-frame estimation, but these models don’t use the entire video sequence during testing. Others rely on optimization-based techniques, which can be time-consuming \cite{semihandobj, liu2022hoi4d}. Finally, some train forward networks like LSTMs \cite{yang2020seqhand,multiviewvideohpe,arctic} or transformers \cite{fu2023deformer} to handle a sequence of frames and predict hand poses. However, these methods generally focus on local pose and 2D alignment, ignoring the global trajectory. Our approach is the first feed-forward method to reconstruct the global trajectory from monocular videos.
\yao{todo: double check methods about depth and optimizaiton. they are mentioned a lot in the intro by yufei, but I actually didn't find good papers for them.}



% \paragraph{4D Whole-Body Pose Estimation.} Feed Forwad:Glamer, WHAM TRACE, Optimization: SLAHMER, PACE etc. Categorize them to optimization based method that relies on learned human motion prior, and feed forward-based methods. Important cues are from human root velocity and foot skating, which is unavailable in hand (our focus). One could first use their method and chop out hand, but they assume a visible full body, which may not hold true. Our global spatial cross-attention can be viewed as an implicit version of this idea.  Furthermore, we show that even if the full body is visible, we are still better. 

\paragraph{4D Whole-Body Pose Estimation.} 
Reconstructing 4D trajectories for the entire human body~\cite{glamr, wham, ye2023decoupling, kocabas2020vibe, kanazawa2019learning, Liu2021_4D, kanazawa2019learning_video, kocabas2020vibe, Choi2021Beyond, Luo2020Motion, Pavlakos2022Human} has garnered significant attention in recent years, with numerous methods proposed for applications in motion capture, animation, and human-computer interaction. These approaches can be broadly categorized into optimization-based methods that rely on learned human motion priors, and feed-forward network-based methods.

Optimization-Based Methods. Optimization-based methods, such as SLAHMR~\cite{slahmr}, PACE~\cite{pace}, and \cite{Sun2021Monocular,Gartner2022Trajectory}, typically obtain camera poses using Structure-from-Motion (SfM) techniques~\cite{Schonberger2016SfM} or SLAM algorithms. They then jointly optimize the camera and human motion by leveraging human motion priors~\cite{Rempe2021HuMoR} to minimize the reprojection error of 2D keypoints and increase the likelihood of the predicted 3D motion. While these methods often achieve high-quality results, they are computationally expensive and may struggle with scenes involving multiple subjects or complex camera movements~\cite{Liu2021_4D}. Additionally, relying solely on local pose information can be insufficient for faithful global trajectory estimation, especially in the presence of occlusions or out-of-distribution poses~\cite{glamr}.

Feed-Forward Methods. Feed-forward approaches have also been explored~\cite{glamr, wham, trace, Li2022DD, Yu2021Human} to directly regress the global trajectory from image features without explicit optimization. For instance, GLAMR~\cite{glamr} adopts a multi-stage pipeline to infer global human trajectories from per-frame local 3D poses, but is vulnerable to occlusions and ignores scene-related information. TRACE~\cite{trace} combines scene information and 3D human motions using a novel 5D representation for end-to-end training, enabling simultaneous estimation of multiple people, yet may lack temporal consistency. WHAM~\cite{wham} fuses 2D keypoints and pixel features, leveraging camera angular velocity and contact information for accurate trajectory estimation, but its performance is constrained by the diversity of motions in the training data.

However, when estimating hand trajectories, the cues used by these whole-body methods, such as root velocity and foot contact, are unavailable. Moreover, the assumption of a visible full body does not hold in videos focusing on hand manipulation, where the body is partially or entirely out of frame. Applying whole-body methods to extract hand motion faces significant challenges due to the lack of full-body visibility and the intricate nature of hand movements. Our approach addresses these limitations by introducing a global spatial cross-attention mechanism that implicitly captures hand motion in global space without relying on body cues. We demonstrate that even when the full body is visible, our method outperforms existing whole-body estimators in reconstructing coherent 4D hand trajectories.




\paragraph{Upgrade Image-Based Models to Videos.} The concept of upgrading pretrained single-image methods to sequence-level through lightweight adaptation has been widely explored in generative AI, particularly for synthesizing coherent objects and scenes. In video generation, image-based generative models~\cite{Karras2019stylegan2,rombach2021highresolution,ding2022cogview2} serve as foundational building blocks for frame-wise generation. These image models are upgrading for video through sequence-level adaptation techniques, including multi-frame hierarchical training~\cite{hong2022cogvideo} , spatiotemporal factorization~\cite{Singer2022MakeAVideoTG}, video noise priors~\cite{Ge2023PreserveYO}, and temporal attention combined with 3D convolutional blocks~\cite{Blattmann2023AlignYL,Blattmann2023StableVD}. In the domain of 3D generation, recent approaches such as MVDream~\cite{Shi2023MVDreamMD}, SyncDreamer~\cite{Liu2023SyncDreamerGM}, and Cat3D~\cite{Gao2024CAT3DCA} similarly extend from pretrained text-to-image (T2I) models, incorporating adaptations to ensure 3D spatial coherence across generated views. Such strategies enable frame-to-frame (view-to-view) consistency while leveraging the frame generation capabilities of T2I models, making them highly efficient compared to training from scratch. 
Drawing inspiration from generative AI approaches, 
% that leverage pretrained image models through lightweight fine-tuning, our work addresses a novel application in 4D hand reconstruction. Specifically, 
we leverages pretrained single-image hand reconstruction models to enable world-coordinate-based hand reconstruction across video sequences with the proposed light-weight adaptation layers. This shift from per-frame to global representation ensures consistent hand reconstruction in a unified coordinate space, enhancing both accuracy and applicability for video-based hand reconstruction.




==> fig/teaser.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/teaser.pdf}
    \caption{\textbf{just a teaser Example \todo{input: } } hamer and ours: all good in overlayed view, then show side view.}
    \label{fig:teaser}
\end{figure*}


% \begin{strip}
% \vspace{-5em}
% \centering
% \includegraphics[width=\linewidth]{fig/teaser.png}
% % \vspace{-0.7cm}
% \captionof{figure}{
% {just a teaser Example} hamer and ours: all good in overlayed view, then show side view.}
% \label{fig:teaser}
% % \vspace{-.2cm}
% \end{strip}


% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{exp/main.pdf}
%     \caption{\todo{change knife to bottle / mugs}}
%     \label{fig:my_label}
% \end{figure*}

==> sec/1_intro_drat.tex <==

\section{Introduction}

% set up the problem: state goal and why global hand trajeotory is important. 
Consider the video frames shown in Figure \ref{fig:teaser}. One can infer not only the articulation of the hand (3D pose) depicted in every  frame but also understand the hand motions across frames and in space. For example, in the first row, we understand that the hand extends towards the drawer and then retracts along a nearly identical path.
The ability to infer 4D hand trajectory (3D space plus time) is important for many downstream tasks, such as reasoning about hand-object interactions in a global scene \cite{ma2022hand}, AR/VR applications \cite{pei2022hand}, and imitation learning in robotics \cite{bharadhwaj2024towards, wang2024dexcap}.
Unfortunately, despite impressive progress in hand pose estimation that infers frame-wise 3D pose, current methods still struggle to coherently put them into a global space. In this work, we address this problem with a system that can infer coherent 4D hand trajectory and pose from monocular videos.


% problem / challenges
While there has been recent interest in estimating 3D body motion in global space \cite{slahmr,glamr,wham,egoego}, such methods do not address the hands, which present unique challenges.
Hands move quickly and are small, meaning that image evidence is often blury or of low resolution. 
Hands are also often partially or fully occluded since they frequently interact with objects, the scene, the other hand, or other body parts. 
Thus tracking hands in 4D is a challenge.

\iffalse
%4D hand trajectories in global space receive less attention despite the growing interest in whole-body trajectory estimation in global space \cite{slahmr,glamr,wham,egoego}. Yet, the problem poses its unique challenges.
% 
First, as the distal part of the body, hand motion depends not only on the root motion but also on the net effect of all joint motions along the kinematic chain. When one uses their hands for interactions or for talking, hand trajectory in space is distinct, and arguably more intricate, than body root trajectory during walking or running.
% 
Second, in videos focusing on hand manipulation, the whole body is often largely truncated, making it infeasible to rely on whole-body pose estimation. 
Besides truncation, occlusions are also very common, either from interacted objects in the scenes or from the other hand or other body parts.
% 
Lastly, hands typically span only 20cm, so they appear small in videos and their intricate motion takes fewer pixels. They often move fast, thus often suffering more from motion blur.
\fi 


% technical background. 
Although \todo{no/?few?} prior works directly predict 4D hand trajectory, there are some common practices that `lift' the per-frame 3D pose outputs from image-based hand pose estimation methods \cite{hamer,frankmocap}. A key step in this process is the estimation of 3D world coordinate of the hand, and the de-facto approach is to leverage a weak-to-full perspective transformation (\wtf), that places the predicted hand at a certain distance given the camera intrinsics and predicted scale (Sec.~\ref{sec:\wtf}). However, we find that this  operation introduces a large error in 4D motion, and that even post-processing optimization struggles to correct it.
% 
With good 2D image alignment, one could infer the depth for each frame to get 4D trajectory. 
% 
Some people set up multiple cameras to triangulate the hands \cite{piano,han,interhand,ho3d}, while 
others obtain depth through estimation \cite{VISOR,egoexo} or depth sensors \cite{arial,liu2022hoi4d}. 
However, occlusions from interacted objects, cluttered scenes, or other body parts hinder accurate hand depth estimation, even with perfect depth sensors.
% 
Finally, video-based feed-forward methods \cite{fu2023deformer,yang2020seqhand, fan2023arctic}, aim to address motion blur and occlusion by fusing features from nearby frames. Nevertheless, their predicted hand poses remain in local cooridnate, and they revert to the aforementioned solutions when recovering 4D trajectory in a global space.

%  our solution: we should learn it
Our insight is that hands do not move arbitrarily in physical space but follow certain motion patterns in daily activities, such as when manipulating objects, talking, or reaching out, \etc. 
We propose to learn this prior directly and predict motion changes in metric space, along with local hand articulation. This results in, to our knowledge, the first feed-forward method that estimates consistent 4D hand trajectories from monocular videos.

% Our solution: idea: lack data --> method (fine-tune and light-weight layers)
The design of our learning system is largely shaped by the limitations posed by training data. Modern learning-based pose estimators~\cite{xu2022vitpose,hmr2,black2023bedlam} benefit from large models like ViTs~\cite{vit} and are notoriously data-hungry. Unfortunately, video datasets with 3D annotations, which should be fueling more data-demanding video models, are much scarcer compared to their image counterparts.
We posit that the heavy lifting happens during inference from pixels to local hand articulation, which can benefit greatly from the learned prior in image-based models, while coherent trajectories can be effectively learned by a modest number of additional inter-connections.
Guided by this insight, we repurpose the state-of-the-art image-based hand pose estimator \cite{hamer} by injecting two types of lightweight attention layers. The first is
a cross-view self-attention that sees across multiple frames to leverage temporal cues. The second is a global-context cross-attention that sees the original frames (from which the input hand images are cropped) to gain a larger field-of-view of the scenes. 
They add merely \todo{xx\%} of new parameters. We finetune the entire network with careful initialization of the new layers. 
Additionally, our model can also be used as single-image pose estimator, allowing us to intersperse both video and image data in training batches, which improves generalization.  


% empirical ruslts 
We evaluate our model \ours~on both allocentric and egocentric videos. We analyze the drawbacks of the prevalent practices, when and why they fail. \ours~significantly outperforms all other potential candidates in terms of global trajectory accuracy. It also provides a better initialization for test-time optimization. 
We carefully ablate our method to analyze our design choices. Notably, when \ours~ serves as an image-based pose estimator, we find that it even outpeforms comparably to the state-of-the-art image-based method in terms of per-frame hand pose accuracy.  
Finally, we show generalization ability to in-the-wild videos and images by presenting more qualitative results. Our model will be publicly released for broader use and further research.




==> table/tab1_exo.tex <==

\definecolor{first}{rgb}{1.0, .83, 0.3}
\definecolor{second}{rgb}{1.0, 0.93, 0.7}
\def \first {\cellcolor{first}}
\def \second {\cellcolor{second}}
\def \third {}

\begin{table*}[t]
\footnotesize
\begin{center}
\vspace{-1em}


\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l l c c c c c c c c c c c }
\toprule
\multirow{2}{*}{Local Pose}& \multirow{2}{*}{Uplift} & \multicolumn{3}{c}{ARCTIC-EXO} 
& \multicolumn{3}{c}{DexYCB} & \multicolumn{3}{c}{ARCTIC-EGO} \\
\cmidrule(r){3-5} \cmidrule(r){6-8} \cmidrule(r){9-11}
 & & GA-MPJPE & FA-MPJPE & ACC-NORM  & GA-MPJPE & FA-MPJPE & ACC-NORM & GA-MPJPE & FA-MPJPE & ACC-NORM   \\
\midrule
HaMeR& \wtf & 7.88 & 21.79 & 81.19 & 3.28 & 12.66 & 14.39 & 2.91 & 5.53 & 11.95 \\
\midrule
HaMeR$\dagger$  & \wtf & 5.53 & 13.29 & 30.09 & 1.93 & 9.78 & 4.42 & 3.48 & 9.23 & 9.62 \\
HaMeR$\dagger$  & \wtf-GT & 6.05 & 15.13 & 36.59 & \second 1.84 & \second 9.48 & 4.27 & \first \textbf{1.84} & \first \textbf{3.66} & 4.39 \\
HaMeR$\dagger$  & ZoeDepth & \second 3.28 & \second 10.09 & \first {1.83} & 4.93 & 20.51 & \first \textbf{1.32} & 2.95 & 5.60 & \first {1.57} \\
HaMeR$\dagger$  & WHAM & 4.79 & 14.41 & 2.43 & -- & -- & -- & -- & -- & -- \\
\multicolumn{2}{c}{\ours$\dagger$ (Ours) } & \first {2.07} & \first {5.18} & \second 2.02 & \first \textbf{1.61} & \first {6.58} & \second 1.82 & \second 2.27 & \second 4.31 & \second 1.58 \\
\midrule
\multicolumn{2}{c}{\ours (Ours)} & \textbf{1.88} & \textbf{4.49} & \textbf{1.48} & 1.80 & \textbf{5.80} & 1.70 & 2.39 & 4.49 & \textbf{1.34} \\
\bottomrule
\end{tabular}
}
\caption{{Comparison with baselines.} We compare our method with different uplifting baselines on two allocentric datasets (ARCTIC-EXO and DexYCB) and one egocentric dataset (ARCTIC-EGO). We report trajectory errors in GA-MPJPE, FA-MPJPE, and ACC-NORM. 
$\dagger$ marks dataset-specific finetuned models on top of publicly released HaMeR while \ours~trains on a combination of datasets. Dark yellow makes the best results and light yellow makes the 2nd best ones among dataset-specific models that trains on the same amount of training data under the same training schedule. Bold text marks the best overall results. } 
\label{tab:compare}
\end{center}
\vspace{-2em}
\end{table*}



==> table/tab1a_arctic.tex <==

% \definecolor{first}{rgb}{1.0, .83, 0.3}
% \definecolor{second}{rgb}{1.0, 0.93, 0.7}
% \def \first {\cellcolor{first}}
% \def \second {\cellcolor{second}}
% \def \third {}

% \begin{table}[t]
% \footnotesize
% \begin{center}
% \vspace{-1em}
% \caption{\textbf{Comparison on Allocentric view of ARCTIC dataset:} GA-MPJPE, GA-ROOT, FA-MPJPE, ACC-NORM, and PA-MPJPE for different models.}
% \vspace{-1em}
% \label{tab:arctic_exo}

% \setlength{\tabcolsep}{2pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l c c c c c}
% \toprule
% method & GA-MPJPE & FA-MPJPE & ACC-NORM & PA-MPJPE \\
% \midrule
% HAMER* & 7.9 & 21.8 & 81.2 & 0.91 \\
% HAMER(GT) & 6.0 & 15.1 & 36.6 & 0.63 \\
% HAMER(U) & 5.5 & 13.3 & 30.1 & 0.63 \\
% ZoeDepth & \second 3.3 & \second 10.1 & \first \textbf{1.8} & 0.63 \\
% WHAM & 4.8 & 14.4 & 2.4 & \todo{0.70} \\
% \ours~(Ours) & \first \textbf{2.1} & \first \textbf{5.2} & \second 2.0 & \first \textbf{0.62} \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \vspace{-2em}
% \end{table}


==> table/tab2_ego.tex <==

% \definecolor{first}{rgb}{1.0, .83, 0.3}
% \definecolor{second}{rgb}{1.0, 0.93, 0.7}
% \def \first {\cellcolor{first}}
% \def \second {\cellcolor{second}}
% \def \third {}

% \begin{table}[t]
% \footnotesize
% \begin{center}
% \caption{\textbf{Comparison on egocentric view of ARCTIC dataset:} GA-MPJPE, GA-ROOT, FA-MPJPE, ACC-NORM, and PA-MPJPE for different models.}
% \label{tab:arctic_exo}

% \setlength{\tabcolsep}{4.5pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l c c c c c}
% \toprule
%  & GA-MPJPE & FA-MPJPE & ACC-NORM & PA-MPJPE \\
% \midrule
% HAMER(GT) & \first \textbf{1.84} & \first \textbf{3.66} & 4.39 & \first \textbf{0.71} \\
% HAMER(U) & 3.48 & 9.23 & 9.62 & \second 0.71 \\
% ZoeDepth & 2.95 & 5.60 & \first \textbf{1.57} & 0.71 \\
% Ours & \second 2.27 & \second 4.31 & \second 1.58 & 0.72 \\
% \midrule
% HAMER* & 2.91 & 5.53 & 11.95 & 0.98 \\
% Ours* & 2.39 & 4.49 & 1.34 & 0.71 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table}
% % 
